Towards Deeper, Lighter and Interpretable Cross Network for CTR Prediction

Click Through Rate (CTR) prediction plays an essential role in recommender systems and online advertising. It is crucial to effectively model feature interactions to improve the prediction performance of CTR models. However, existing methods face three significant challenges. First, while most methods can automatically capture high-order feature interactions, their performance tends to diminish as the order of feature interactions increases. Second, existing methods lack the ability to provide convincing interpretations of the prediction results, especially for high-order feature interactions, which limits the trustworthiness of their predictions. Third, many methods suffer from the presence of redundant parameters, particularly in the embedding layer. This paper proposes a novel method called Gated Deep Cross Network (GDCN) and a Field-level Dimension Optimization (FDO) approach to address these challenges. As the core structure of GDCN, Gated Cross Network (GCN) captures explicit high-order feature interactions and dynamically filters important interactions with an information gate in each order. Additionally, we use the FDO approach to learn condensed dimensions for each field based on their importance. Comprehensive experiments on five datasets demonstrate the effectiveness, superiority and interpretability of GDCN. Moreover, we verify the effectiveness of FDO in learning various dimensions and reducing model parameters. The code is available on \url{https://github.com/anonctr/GDCN}.

==> copy.tex <==
\begin{table*}
\centering
\caption{Results of parallel models, which integrates Implicit Feature Interactions, i.e., DNN module.}
\label{tab:all}
\scalebox{0.95}{
\begin{tabular}{cc|cc|cc|cc|cc|cc|cc} 
\hline
\hline
 &Datasets  & \multicolumn{2}{c|}{Criteo} & \multicolumn{2}{c|}{Avazu}& \multicolumn{2}{c|}{Malware} & \multicolumn{2}{c|}{Frappe} & \multicolumn{2}{c|}{ML-tag} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\Delta{AUC} $\\ $\uparrow$\end{tabular}} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\Delta{Logloss} $\\$\downarrow$\end{tabular}}} \\ 
\cline{1-12}
Model & Operations & AUC & Logloss & AUC & Logloss& AUC & Logloss & AUC & Logloss & AUC & Logloss &  & \\ 
\hline
WDL & LR, DNN & 0.8130 & 0.4386 & 0.7877 & 0.3758 && & 0.9790 & 0.1652 & 0.9595 & 0.2859 &  &  \\
DCN & CN, DNN & 0.8141 & 0.4378 & 0.7890 & 0.3745 &&& 0.9797 & 0.1618 & 0.9601 & 0.2299 &  &  \\
DeepFM & FM, DNN & 0.8137 & 0.4382 & 0.7891 & 0.3745 &&& 0.9801 & 0.1680 & 0.9595 & 0.2440 &  &  \\
xDeepFM & CIN, DNN & 0.8142 & 0.4377 & 0.7893 & 0.3742 &&& 0.9805 & 0.1656 & 0.9598 & 0.2330 &  &  \\
AutoInt+ & Autoint, DNN & 0.8144 & 0.4376 & 0.7889 & 0.3745 &&& 0.9802 & 0.1654 & 0.9610 & 0.2345 &  &  \\
AFN+ & AFN, DNN & 0.8138 & 0.4384 & 0.7883 & 0.3749 &&& 0.9807 & 0.1620 & 0.9605 & 0.2281 &  &  \\
DCN-V2 & CN2, DNN & 0.8144 & 0.4375 & 0.7898 & 0.3743 &&& 0.9809 & 0.1539 & 0.9603 & 0.2284 &  &  \\ 
\hline
NON &LR, Att., DNN  & 0.8133 & 0.4390 & 0.7889 & 0.3747&& & 0.9787 & 0.1700 &0.9609	&0.2279 &  &  \\
FED &Concat, Att., DNN & 0.8141 & 0.4379 & 0.7891 & 0.3745&& & 0.9804 & 0.1616 & 0.9610 & 0.2294 &  &  \\ 
\hline
DGCN-P & GCN DNN & 0.8161 & 0.4360 & 0.7909 & 0.3734&& & 0.9842 & 0.1410 & 0.9663 & 0.2144 &  &  \\
 & \textit{Imp.} & 0.0018 & -0.0016 & 0.0011 & -0.0009 &&& 0.0032 & -0.0116 & 0.0053 & -0.0150 &  &  \\
\hline
\bottomrule
\end{tabular}
}
\end{table*}




\begin{table}
    % \setlength{\abovecaptionskip}{0.2cm}
    % \setlength{\belowcaptionskip}{-0.2cm}
\centering
\caption{Optimized dimension of each field in Criteo, 95\% and 90\% variance kept. $\hat{D}$ indicates weighted average dimension of all features. And $\overline{K}$ is the arithmetic average dimension of all fields in one instance.}
\label{tab:80_90}
\scalebox{0.9}{
\begin{tabular}{c|ccccc|cccc} 
\hline
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Field \\ID\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Feat.\\Num\end{tabular}} & \multicolumn{2}{c}{\textbf{ Emb Dim}} & \multirow{2}{*}{For.} & \multicolumn{1}{r}{\multirow{2}{*}{\begin{tabular}[c]{@{}r@{}}Field \\ID\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Feat.\\Num\end{tabular}}} & \multicolumn{1}{c}{\textbf{\textbf{Emb Dim}}} & \multicolumn{1}{l}{} & \multirow{2}{*}{For.} \\ 
\cline{3-4}\cline{8-8}
 &  & 95\% & 80\% &  & \multicolumn{1}{r}{} & \multicolumn{1}{c|}{} & 80\% & \multicolumn{1}{l}{} &  \\ 
\hline
\#1 & 49 & 5 & 2 & 2 & \#22 & 4 & 2 & 2 & 1 \\
\#2 & 101 & 13 & 8 & 3 & \#23 & 42,646 & 15 & 10 & 14 \\
\#3 & 126 & 7 & 3 & 3 & \#24 & 5,178 & 14 & 10 & 8 \\
\#4 & 45 & 4 & 2 & 2 & \#25 & 192,773 & 2 & 2 & 20 \\
\#5 & 223 & 13 & 7 & 3 & \#26 & 3,175 & 13 & 9 & 7 \\
\#6 & 118 & 9 & 4 & 3 & \#27 & 27 & 4 & 3 & 2 \\
\#7 & 84 & 8 & 3 & 3 & \#28 & 11,422 & 13 & 9 & 10 \\
\#8 & 76 & 5 & 2 & 2 & \#29 & 181,075 & 5 & 4 & 20 \\
\#9 & 95 & 9 & 3 & 3 & \#30 & 11 & 5 & 4 & 1 \\
\#10 & 9 & 4 & 2 & 1 & \#31 & 4,654 & 12 & 8 & 8 \\
\#11 & 30 & 3 & 2 & 2 & \#32 & 2,032 & 11 & 7 & 6 \\
\#12 & 40 & 4 & 2 & 2 & \#33 & 5 & 3 & 2 & 1 \\
\#13 & 75 & 4 & 2 & 2 & \#34 & 189,657 & 5 & 2 & 20 \\
\#14 & 1,458 & 12 & 8 & 6 & \#35 & 18 & 5 & 4 & 2 \\
\#15 & 555 & 12 & 5 & 4 & \#36 & 16 & 7 & 4 & 2 \\
\#16 & 193,949 & 4 & 3 & 20 & \#37 & 59,697 & 11 & 8 & 15 \\
\#17 & 138,801 & 8 & 5 & 19 & \#38 & 86 & 5 & 3 & 3 \\
\#18 & 306 & 10 & 6 & 4 & \#39 & 45,571 & 10 & 6 & 14 \\ 
\cline{6-10}
\#19 & 19 & 6 & 4 & 2 & \multicolumn{5}{c}{} \\ 
\cline{10-10}
\#20 & 11,970 & 14 & 10 & 10 & \multicolumn{2}{r}{Weighted Ave. $\overline{D}$} & \multicolumn{1}{l}{5.92} & 3.98 &  \\ 
\cline{10-10}
\#21 & 634 & 11 & 6 & 5 & \multicolumn{2}{r}{Arithmetic Ave. $\overline{K}$} & \multicolumn{1}{l}{7.87} & 4.85 &  \\
\hline
\hline
\end{tabular}
}
\end{table}


% \begin{table}
% \centering
% \caption{The comparison of three different dimension assigning methods.}
% \label{tab:3 ways}
% \begin{tabular}{c|ccccc} 
% \toprule
% Models & CN-V2 & GCN & DNN & DCN-V2 & GDCN-P \\ 
% \hline
% Fixed & 0.8141 & 0.8154 & 0.8141 & 0.8144 & 0.8161 \\
% 95 & 0.8142 & 0.8157 & 0.8140 & 0.8143 & 0.8160 \\
% 80 & 0.8140 & 0.8155 & 0.8135 & 0.8140 & 0.8158 \\
% Formula & 0.8139 & 0.8155 & 0.8136 & 0.8140 & 0.8157 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \usepackage{booktabs}


\begin{table}
\centering
\caption{The comparison of three different dimension assigning methods.}
\label{tab:3 ways}
\begin{tabular}{c|ccccc} 
\toprule
Models & CN-V2 & GCN & DNN & DCN-V2 & GDCN-P \\ 
\hline
Fixed & \begin{tabular}[c]{@{}c@{}}0.8141\\(18.6M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8154\\(19.7M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8141\\(18.0M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8144\\(19.1M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8161\\(20.3M)\end{tabular} \\ 
\hline
FDO(95\%) & \begin{tabular}[c]{@{}c@{}}0.8142\\(6.7M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8157\\(7.0M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8140\\(12.2M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8143\\(10.95M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8160\\(7.4M)\end{tabular} \\ 
\hline
Formula & \begin{tabular}[c]{@{}c@{}}0.8139\\(21.6M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8154\\(21.9M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8136\\(21.8M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8140\\(22.1M)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8157\\(22.3M)\end{tabular} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{The comparison of three different dimension assigning methods.}
\label{tab:3 ways}
\begin{tabular}{c|ccccc} 
\toprule
Models & CN-V2 & GCN & DNN & DCN-V2 & GDCN-P \\ 
\hline
Fixed & 0.8141 & 0.8154 & 0.8141 & 0.8144 & 0.8161 \\
FDO(95\%) & 0.8142 & 0.8157 & 0.8140 & 0.8143 & 0.8160 \\
Formula & 0.8139 & 0.8154 & 0.8136 & 0.8140 & 0.8157 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table*}
    \setlength{\abovecaptionskip}{0.2cm}
    \setlength{\belowcaptionskip}{-0.2cm}
\centering
\caption{Results of parallel models, which integrates implicit feature interactions, i.e., DNN network. We list the main parallel networks for each model. And we calculate the $\Delta{AUC}$ and $\Delta{Logloss}$ compared to the vanilla DNN model.}
\label{tab:parallel}
\scalebox{0.85}{
\begin{tabular}{r|cc|cc|cc|cc|cc|cc} 
\hline
\hline
 Datasets  & \multicolumn{2}{c|}{Criteo} & \multicolumn{2}{c|}{Avazu}& \multicolumn{2}{c|}{Malware} & \multicolumn{2}{c|}{Frappe} & \multicolumn{2}{c|}{ML-tag} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\Delta{AUC} $\\ $\uparrow$\end{tabular}} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\Delta{LL} $\\$\downarrow$\end{tabular}}} \\ 
\cline{1-11}
Model(Networks) & AUC & Logloss & AUC & Logloss& AUC & Logloss & AUC & Logloss & AUC & Logloss &  & \\ 
\hline
DNN & 0.8139 & 0.4383 & 0.7886 & 0.3748 &0.7424 & 0.5928& 0.9794 & 0.1661 & 0.9598 & 0.2418 & - &-  \\
\hline
WDL(LR, DNN) & 0.8141 & 0.4379 & 0.7888 & 0.3747 &0.7436 & 0.5915& 0.9801 & 0.1652 & 0.9605 & 0.2411 & 0.07\%	&-0.23\%  \\
DeepFM(FM, DNN) & 0.8140 & 0.4378 & 0.7891 & 0.3745 &0.7424 & 0.5925& 0.9808 & 0.1613 & 0.9606 & 0.2440 &  0.05\%	&-0.42\%  \\
DCN(CN, DNN) & 0.8142 & 0.4378 & 0.7890 & 0.3745 &0.7434&0.5917& 0.9805 & 0.1618 & 0.9607 & 0.2283 &  0.08\%	&-1.69\%  \\
xDeepFM(CIN, DNN) & 0.8142 & 0.4377 & 0.7893 & 0.3744 &\underline{0.7442} & \underline{0.5911} & 0.9806 & 0.1638 & 0.9609 & 0.2328 &  0.12\%	&-1.12\%  \\
AutoInt+(Autoint, DNN) & \underline{0.8144} & 0.4376 & 0.7886 & 0.3745 &0.7435 & 0.5917& 0.9802 & 0.1654 & 0.9609 & 0.2343 &  0.07\%	&-0.76\%  \\
AFN+(AFN, DNN) & 0.8138 & 0.4384 & 0.7887 & 0.3748 &0.7439&0.5912& 0.9807 & 0.1620 & 0.9605 & 0.2295 &  0.07\%	&-1.53\%  \\
DCN-V2(CN-V2, DNN) &\underline{0.8144} & \underline{0.4375} & \underline{0.7898} & \underline{0.3743} &0.7433 & 0.5920&0.9810 & \underline{0.1539} & 0.9603 & 0.2284 &  0.11\%	&-2.67\%  \\ 

\hline
NON(LR, Att., DNN)  & 0.8133 & 0.4390 & 0.7889 & 0.3747&0.7426 & 0.5925 & 0.9803 & 0.1564 &0.9609	&0.2279 &  0.03\%	&-2.26\%  \\
FED(Concat, Att., DNN) & 0.8141 & 0.4379 & 0.7891 & 0.3745&0.7436 & 0.5915&\underline{0.9811} & 0.1590 & \underline{0.9610} & 0.2294 & 0.12\%	&-1.99\%  \\ 
ParaMaskNet(MaskBlocks, DNN) &0.8142&0.4377  &0.7895 & 0.3748  &0.7435& 0.5920  &0.9805 &0.1559   &0.9608 &\underline{0.2272}   &0.10\% 	&-2.47\%\\
\hline
GDCN-P(GCN, DNN) &\textbf{0.8161} & \textbf{0.4360} & \textbf{0.7909} & \textbf{0.3734}&\textbf{0.7462} &\textbf{0.5893}&\textbf{0.9842} & \textbf{0.1410} & \textbf{0.9663} & \textbf{0.2144} &  \textbf{0.44\%}	&\textbf{-5.57\%}  \\
\textit{Rel.Imp}  & 0.0017 & -0.0015 & 0.0011 & -0.0009 &0.0020&-0.0018& 0.0031 & -0.0129 & 0.0053 & -0.0128 &- & -\\
% 0.40%	-4.54%

\hline
\bottomrule
\end{tabular}
}
\end{table*}


\subsubsection{The understanding of independent field dimensions.}  The field dimension learned by the FDO indicates the importance of the corresponding field. Figure \ref{fig:10w_gate values} counts the averaged field-level gate vectors on 100,000 input instances. Overall, important crossing features decrease sharply as the number of cross layers rises. Each color block reflects the importance of each field, especially in the 1st order, e.g., field \{\#20, \#23,\#24 \} is important(red block) but field \{\#11, \#27, \#30\} are unimportant(blue block). Return to Table \ref{tab:80_90}, field \{\#20, \#23,\#24\} exactly have the longer dimension after applying FDO with 95\% variance. Conversely, field \{\#11, \#27, \#30\} have the shorter dimension. We further compute the Pearson Correlation Coefficient between the averaged field-level gate vector in 1st order and the optimization field dimensions with 95\% variance, which is 0.79 with p-value<1*e-9. It verifies the significant correlation between the field dimension and the importance of corresponding field. Field importance information is retained in the embedding table, and FDO successfully learns it from the embedding table. Hence, we can identify which fields are important directly from the field dimensions learned by FDO. Furthermore, the field dimension is not always related to the feature number in the field. For example, field \{\#16, \#25\} has the most feature number, but their field dimension is short, and their importance is also insignificant. However, when adopting the Formula method to assign field dimension, field \{\#16, \#25\} would have the longest dimension. Hence, this also indicates the rationality and superiority of the proposed FDO approach.
